Is thermography a viable solution for detecting pressure injuries in dark skin patients?

Pressure injury (PI) detection is challenging, especially in dark skin tones, due to the unreliability of visual inspection. Thermography has been suggested as a viable alternative as temperature differences in the skin can indicate impending tissue damage. Although deep learning models have demonstrated considerable promise toward reliably detecting PI, the existing work fails to evaluate the performance on darker skin tones and varying data collection protocols. In this paper, we introduce a new thermal and optical imaging dataset of 35 participants focused on darker skin tones where temperature differences are induced through cooling and cupping protocols. We vary the image collection process to include different cameras, lighting, patient pose, and camera distance. We compare the performance of a small convolutional neural network (CNN) trained on either the thermal or the optical images on all skin tones. Our preliminary results suggest that thermography-based CNN is robust to data collection protocols for all skin tones.

==> 4_Related_work.tex <==
Pandey et al\citep{pandey2022deep} proposed an automated approach for detecting pressure ulcers using thermal images and deep learning techniques to segment the region of  pressure ulcer  with surrounding healthy tissue. Their study involved 10 subjects with pressure ulcers at various stages.Using a FLIR E60 camera mounted on a tripod,images were captured with the ulcers directly facing the camera. An  SSD MobileNet V2 object detection model, initially trained on the COCO 2017 dataset\citep{caesar2018coco}  was used and fine-tuned using 15 of their 18 collected images.The remaining 3 images were used for testing. However,their approach is limited by the small dataset size and did not account for variations in lighting conditions or camera distance. 

Wang etal \citep{wang2021infrared} proposed a a Convolutional Neural Network approach for classifying infrared thermal images.Using FLIR One Pro camera, images were collected from 349 patients over a period of 10 days.A total of 82 infrared pressure injury and control images were captured, which was used for model training. For testing,images of patients were captured one day before the pressure ulcers were recorded. Authors assumed these  testing images could have pressure injury.Images were captured with patients in the 90\circ lateral position, exposing the area required
for the sacral region and lower back completely.
Leveraging pre-trained CNN (LeNet\citep{lecun1998gradient},AlexNet\citep{krizhevsky2017imagenet},VGGNet\citep{karen2014very}) and  ML models(Random Forest,SVM)images were classified. An accuracy of 95.2\%  and AUC of 0.98 was acheived by the CNN models, which indicates its potential in pressure injury detection. However, variation in skin tone of subjects was not reported.It is also unknown how images  of the ulcers taken at different angles could affects classification accuracy.

==> Archive/1_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
A pressure injury (PI) refers to ``localized damage to the skin and underlying soft tissue, usually occurring over a bony prominence or related to medical devices" \citep{mondragon2024pressure}. 
It continues to be a major issue with at least 1 in 10 adults admitted to the hospital developing a PI \citep{li2020global}.
Furthermore, PI is linked to a decline in quality of life \citep{khor2014determinants}, increased mortality rates \citep{bergquist2013pressure}, extended hospital stays, and a higher likelihood of requiring institutional care after discharge. 
Identifying warning signs of PI can lead to effective preventive actions and early interventions \citep{jiang2020skin,baron2022efficacy}. 

% These injuries to the skin and soft tissues continue to be a major issue in hospitals and long-term care facilities,and are linked to a decline in quality of life\citep{khor2014determinants}, increased mortality rates\citep{bergquist2013pressure}, extended hospital stays, and a higher likelihood of requiring institutional care after discharge. The economic burden posed by pressure injury is a contributing factor to rising healthcare costs\citep{dreyfus2018assessment}. Estimates vary widely \citep{bergquist2013pressure,dreyfus2018assessment,mallah2015effectiveness,reddy2006preventing,padula2019national},but seem to be growing steadily over time. The Agency for Healthcare Research and Quality (AHRQ) estimates HAPI costs at \$10 billion each year, while other cost estimates indicates that the  costs in the US may exceed \$26.8 billion \citep{reddy2006preventing,padula2019national}. Hospital-acquired pressure  injuries(HAPIs) are also responsible for around 60,000 deaths each year, ranking as the eighth leading cause of death in the U.S.\citep{padula2019national}. 

Contemporary techniques for assessing PI risk include using the Braden Scale \citep{bergstrom1987braden,borghardt2015evaluation} and visual inspection. Visual inspection includes assessing the skin for temperature variations, changes in tissue consistency, and the presence of tenderness.
Yet visual inspection for dark skin tone patients is especially challenging and has led to racial disparities in PI outcomes \citep{black2023current}.
As such, alternative technological approaches have been explored for PI detection including thermography (i.e., thermal imaging) \citep{moore2022measuring,jiang2022application}.
% When evaluating skin temperature, a noticeable difference between the region of interest and the surrounding skin can signal a developing pressure injury\citep{farid2012using,edsberg2016revised}.
% Increased warmth might suggest inflammation, while cooler areas could indicate reduced blood circulation.The texture of the tissue also provides valuable information\citep{epuap_npuap_pppia_2019}. Unusual firmness in the assessed area may point to underlying deep tissue damage\citep{defloor2004inter}. Conversely, a spongy or boggy texture could be a sign of edema or fluid accumulation\citep{bryant2015acute}. Tenderness or pain upon palpation of the area is also another important clinical sign \citep{bergstrom1987braden}.      Increased sensitivity in a particular region can serve as an early warning sign of tissue damage and should be considered a risk factor for pressure injury development.
Additionally, researchers have explored various technological approaches for pressure injury (PI) detection,including thermal imaging (thermography), ultrasound, spectroscopy, laser Doppler, and sub-epidermal moisture measurement (SEMM) \citep{gefen2020modelling,oliveira2017accuracy,scafide2020bedside,gefen2018observational,moore2022measuring}. SEMM is currently considered the most advanced method and is recommended in the NPIAP Clinical Practice Guidelines\citep{epuap_npuap_pppia_2019}.However, these devices are costly, with estimates ranging from \$5,000 to \$10,000 per unit, and have not been extensively tested on individuals with darker skin tones\citep{gefen2020modelling,scafide2020bedside,gefen2018observational}. Furthermore, SEMM requires direct skin contact, potentially increasing infection risk through microbial fomite transfer from the device. Thermography offers an alternative approach in the form of expensive, EMR-integrated systems and more affordable off-the-shelf thermal cameras estimated at \$450 per unit). These devices generate color-mapped images of skin temperature, which necessitate either post-processing or qualitative interpretation by healthcare professionals. Research shows that temperature disparities between an area of interest and a control region caused by temperature abnormalities from partial or complete capillary occlusion at compression sites\citep{wang2021infrared,bennett2017long} can indicate impending tissue damage before visual signs appear\citep{moore2022measuring,jiang2022application}.Nonetheless, limited research has been conducted on the relationship between thermal imaging effectiveness and underlying skin tone\citep{sprigle2003analysis,house2015repeatability}. Moreover, a survey of nurses revealed difficulties in integrating thermography into clinical practice, partly due to challenges in data interpretation\citep{sprigle2003analysis}. Aside the cost of these devices, detecting PI on dark skin is problematic since most PI assessment are performed visually, which can be a unreliable and difficult process\citep{zhang2021examining}.
The objective of this study to develop a system capable of detecting pressure injuries on individuals with dark skin tones across various patient positions and lighting conditions. We investigate the feasibility of identifying pressure injuries in patients with darker skin complexions while they are positioned in different orientations and under diverse illumination scenarios. We examine how the distance at which thermal images are captured affects the system's detection accuracy. Our approach involves fine-tuning pre-trained convolutional neural networks (CNNs) using our custom-collected dataset, and evaluating their efficacy in detecting pressure injuries across the diverse dark skin tones represented in our data.
The key contributions of this research are as follows:
i) compilation of a dataset comprising of optical and thermal images from 35 patients with dark skin tones who participated in this study.
ii) evaluation of various pre-trained CNN models' capabilities in identifying pressure injuries from these images.
iii) analysis of how patient positioning and lighting conditions impact thermography data in a controlled clinical simulation environment.iv) development, assessment, and refinement of a protocol for daily thermography data collection on high-risk patients with dark skin tones under typical clinical environmental conditions.

==> Archive/2_Method.tex <==
\section{Method}

\subsection{Data Collection}
\label{sec:data_collection}
Our IRB-approved study collected optical and thermal images from 35 healthy adults.\footnote{To preserve anonymity, the IRB institution and number are omitted but will be provided in the accepted version.} 30 participants had darker skin tones (Monk Skin Tone Scale level 6 or greater) and 5 had lighter skin tones (Monk Skin Tone Scale level 5 or lower). Using a digital colorimeter, we categorized the skin tone of subjects into InterLow, Inter, InterMid, and InterHigh categories as shown in Figure \ref{fig:image_example}. The lower back of each participant was marked to conduct both a cooling and cupping protocol separately. The cooling protocol involved a cooled stone cylinder placed on the right lower back. The cupping protocol was performed using a device to induce erythema (i.e., abnormal redness of the skin).

Images were taken with 2 thermal imaging cameras, the FLIR E8-XT (320x240 resolution) and the FLIR Pro One (160×120 resolution). 
For the cooling protocol, the imaging collection protocol was varied to capture (i) two lighting settings (i.e., ambient and ring light), (ii) two distances (i.e., 35 and 50 cm), and (iii) three different postures (i.e., forward placement of top knee, knees stacked, backward placement of top knee).
For the cupping protocol, we used only the FLIR E8-XT at a single acquisition setting (50 cm and knees stacked).
Each subject had a total of 59 images.
A total of 1680 images were taken during the cooling and control (or base) conditions.
Additionally, 314 images were captured to document erythema.



% The study concluded with a total of 59 images per subject, 2 control images, 48 pre-post paired cooled images, and 9 cupping(erythema) images captured under systematically varied lighting and positioning parameters. The study collected a comprehensive set of images: 1680 images were taken during cooling and control (base) conditions, collectively referred to as the cooling dataset. Additionally, 314 images were captured to document erythema, forming the erythema dataset.

% each at 2 distances and 2 different lighting settings (ring light or room light). 
% Based on this, we categorized the skin tone of subjects into  FLIR E8-XT and the FLIR Pro One were used to capture the optical and thermal images of the sacral region using the Multi-Spectral Dynamic Imaging (MSX) setting , allowing the visual and thermal image to be seen in a single fusion image. The study excluded individuals under 18, pregnant women, and those with certain skin conditions or bleeding disorders. 
% This comprehensive approach aimed to improve erythema detection across various skin tones, addressing a gap in current medical assessment tools.
% The  posterior sacral iliac spines (PSIS) of participants were marked  for conducted  cooling and cupping protocols. The cooling protocol involves placing a stone cylinder cooled at $60^\circ$F on the right PSIS for five minutes, while cupping was performed on the left PSIS to induce erythema. Control images were taken using thermal cameras with participants in side-lying position. Images were captured under varied conditions: two lighting settings (ambient and controlled), two distances (50cm and 35cm), and three postures (side-lying with legs on top of one another and pillow between knees (knees stacked), side lying with forward placement of top knee, creating an increase in flexion of the top hip (knee forward) and side-lying with rearward placement top knee, creating a decrease in flexion of top hip (knee behind). This resulted in a total of 12 protocols. Images of each subject was taken using these 12 protocols. Cupping(inducing erythema) and cooling procedures were followed by imaging series in specific positions and lighting conditions. The study concluded with a total of 59 images per subject, 2 control images, 48 pre-post paired cooled images, and 9 cupping(erythema) images captured under systematically varied lighting and positioning parameters. The study collected a comprehensive set of images: 1680 images were taken during cooling and control (base) conditions, collectively referred to as the cooling dataset. Additionally, 314 images were captured to document erythema, forming the erythema dataset.


% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{Themal_imaging_pics/Optical_diff_skin_tones.png}
%     \caption{Control optical images of different skin tones with the posterior sacral iliac spines (PSIS) marked.}
%     \label{fig:skin-tones-optical}
% \end{figure*}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width = \textwidth]{Themal_imaging_pics/Thermal_diff_skin_tones.png}
%     \caption{Control thermal images of different skin tones}
%     \label{fig:skin-tones-thermal-color}
% \end{figure*}

\subsection{Deep Learning Models}
Convolutional neural networks (CNNs), have revolutionized image analysis and classification tasks in recent years \citep{lecun2015deep}. These models have demonstrated remarkable performance in various medical imaging applications, including dermatological assessments \citep{esteva2017dermatologist}. 

% Among the efficient CNN architectures, MobileNetV2 stands out for its balance of accuracy and computational efficiency, making it suitable for deployment on resource-constrained devices\citep{sandler2018mobilenetv2}.

We used MobileNetV2 for this study. MobileNetV2 typically consists of an initial fully convolutional layer with 32 filters, followed by 19 residual bottleneck layers, and concludes with a 1x1 convolution, global average pooling, and a final fully connected layer\citep{sandler2018mobilenetv2}. The model's efficiency and effectiveness make it a promising candidate for real-time pressure injury detection systems, particularly in scenarios where computational resources may be limited, such as in portable devices used for bedside assessments \citep{howard2019searching}.



% MobileNetV2 builds upon its predecessor by introducing inverted residuals and linear bottlenecks, which significantly reduce the number of parameters while maintaining high accuracy\citep{sandler2018mobilenetv2}.This architecture has been successfully applied in various medical imaging tasks, such as skin lesion classification\citep{mahbod2020transfer} and wound assessment\citep{wang2020deep}.The model's efficiency and effectiveness make it a promising candidate for real-time pressure injury detection systems, particularly in scenarios where computational resources may be limited, such as in portable devices used for bedside assessments\citep{howard2019searching}.

\subsection*{Pressure Injury Classification}

Data is split randomly into training and test set with 80\% for training and 20\% for testing as shown in Table 1. To have a fair basis for comparison, we ensure that we have the same images in the train and test splits across the three cooling and Base dataset. For instance, if image 1 is in the training data of optical images dataset, the corresponding image 1 of thermal colored and thermal black and white will be in their respectively training data. We do the same for training and test data in erythema dataset too. Next, we split the images into 80\% training and 20\% testing. We perform 5-fold cross-validation with the training data, using 4 folds for training and 1 fold for validation as shown in Figure \ref{fig:model}. All the images resized to 224*224 pixels before feeding them as inputs to a deep learning model during training and testing. We employed data augmentation, which is commonly used in deep learning during training to prevent over-fitting of the models, and to increase the model's generalizablilty. Augmentations used are horizontal flip and random rotation.For horizontal flip, images were flipped horizontally, while for random  rotation, images were rotated at 20 degrees. Rotation helps the model to become invariant of object orientation. Following argumentation was image normalization. Both train and test images were normalized with mean of [0.485, 0.456, 0.406] and standard deviation of [0.229, 0.224, 0.225]. The best model based on the highest validation accuracy over the 5-fold cross-validation was selected and finally used to classify the images in the test set.  

% \begin{table}[htbp]
% \floatconts
%   {tab:}
%   {\caption{Number of train and test samples for Erythema and Cool/Base images}}%
%   {\begin{tabular}{p{2.2cm}p{2.3cm}cc}
%     \toprule
%     & \textbf{\# Samples} & \textbf{Train} & \textbf{Test} &  \\
%     \midrule
%     Cool/Base Images & Optical, B\&W thermal, Color thermal & 1337 &343 \\
%     \addlinespace
%     Erythema & Optical, B\&W thermal, Color thermal & 251 & 63  \\
%     \bottomrule
%   \end{tabular}}
% \end{table}

\begin{table}[h]
\floatconts
  {tab:samples} % Label for the table
  {\caption{Number of train and test samples for Erythema and Cool/Base images}} % Caption for the table
  {\centering % Center the table
  \begin{tabular}{p{2.2cm}p{2.3cm}cc}
    \toprule
    & \textbf{\# Samples} & \textbf{Train} & \textbf{Test} \\
    \midrule
    Cool/Base Images & Optical, B\&W thermal, Color thermal & 1337 & 343 \\
    \addlinespace
    Erythema & Optical, B\&W thermal, Color thermal & 251 & 63 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

Our system was implemented using Python, leveraging the PyTorch framework \citep{paszke2019pytorch} for deep learning operations. We utilized additional libraries including Numpy \citep{harris2020array} for numerical computations and Matplotlib \citep{hunter2007matplotlib} for data visualization, and OpenCV \citep{bradski2000opencv} for image processing tasks. The development was carried out in Visual Studio Code.





\subsection*{Model Hyperparameters }

The models used were trained with the same hyperparameters: (a) batch size of 32,(b) 50 epochs,and (c) learning rate of \(1\times e^{-3}\) and (d) early stopping (patience of 10). Also, each model used the Adam optimizer\citep{kingma2020method}and binary cross entropy loss function. The Adam optimizer is a stochastic gradient descent approach that uses adaptive estimates of first-order and second-order moments. The best model based on highest validation accuracy was saved and used for classification on the test set. We used the ImageNet\citep{russakovsky2015imagenet} pre-trained model for fine-tuning to speed up the model convergence and improve the overall classification accuracy.

\subsection*{Performance Metrics}

Our study focuses on a binary classification task across our two datasets. For the Cooling dataset, we aim to categorize images into either the cool (positive class) or the base(negative class). Similarly, for the Erythema dataset, our objective is to classify input images as either erythema(positive class) or base (negative class).

In our evaluation process, we employ the fundamental concepts of classification performance
% \begin{itemize}
%     \item True positives (\(T_p)\): Correctly identified Cool/Erythema images
%     \item True negatives (\(T_n)\): Correctly identified Base images
%     \item False positives (\(F_p)\): Base images incorrectly classified as Cool/Erythema
%     \item  False negatives (\(F_n)\): Cool/Erythema images incorrectly classified as Base
% \end{itemize}
A true positive (\(T_p)\)represents an image that is actually Cool/Erythema and is correctly classified as such by our model. Conversely, a false negative (\(F_n)\) occurs when an image that is truly Cool/Erythema is mistakenly categorized as Base by the model.
Performance metrics used are accuracy, sensitivity, specificity, F1-score, and AUROC. These metrics provide a multifaceted evaluation of each model's classification capabilities.
Accuracy represents the proportion of correct predictions (both true positives and true negatives) among the total number of cases examined.


By examining these diverse metrics (as shown in Table 2), we can gain a comprehensive understanding of each model's strengths and weaknesses across different aspects of classification performance. This multi-metric approach allows for a more nuanced comparison between models and helps in selecting the most appropriate model for our classification task.

==> Archive/3_Results.tex <==

\section*{Results}

\subsection*{Evaluation results}

The implementation of MobileNetV2 yielded promising results across various imaging modalities for skin condition classification as shown in Table \ref{tab:mobilenet_results}. For the cooling dataset, both thermal imaging techniques (black \& white and color) achieved perfect performance with an accuracy and AUC of 1.0000, significantly outperforming the optical imaging which recorded an accuracy of 0.7085 and an AUC of 0.8181. 
In the erythema detection task, both thermal color imaging and black and white thermal imaging demonstrated the highest accuracy at 0.8889, while optical imaging showed an accuracy of 0.8413. 
% Interestingly, for erythema detection, optical imaging exhibited a competitive AUC of 0.9092, surpassing both thermal modalities (B&W: 0.9380, Color: 0.9348). These results suggest that while thermal imaging excels in cool/base classification, the choice of optimal modality for erythema detection may depend on the specific performance metric prioritized. 
The consistently high performance of thermal imaging across both tasks underscores its potential as a robust tool for skin condition assessment when coupled with the MobileNetV2 architecture. 
\begin{table}[htbp]
\floatconts
  {tab:mobilenet_results}%
  {\caption{Comparing performance across 2 tasks and image modalities for MobileNetV2.}}%
{\vspace{-20pt} \scriptsize
  \begin{tabular}{l l l l l }
\toprule
\textbf{Task} & \textbf{Image} & F1 & AUC \\
\midrule
 & Optical & 0.711 & 0.818 \\
Cooling & Thermal (B\&W) & 1.000 & 1.000 \\
& Thermal Color & 1.000 & 1.000 \\
\midrule
& Optical  & 0.8684 & 0.9092 \\
Erythema  & Thermal (B\&W)  & 0.9136 & 0.9380 \\
& Thermal (Color) & 0.9176 & 0.9348 \\
\bottomrule
\end{tabular}}
%   {\begin{tabular}{p{2cm} p{2cm} p{2cm} p{1.8cm} p{1.8cm} p{1.9cm} p{1.8cm} } 
% \toprule
%   \bfseries{Performance Metrics}&
%   \bfseries{Optical} & \bfseries{Thermal B\&W} & \bfseries{Thermal Color} & \bfseries{Optical Erythema} & \bfseries{Thermal B\&W Erythema} & \bfseries{Thermal Color Erythema} \\
% \midrule
% Accuracy & 0.7085
% & \textbf{1.0000} & \textbf{1.0000}&0.8413 & \textbf{0.8889} & 0.8889\\ 
% Sensitivity & 0.7278& 1.0000 & 1.0000 & 0.8250& 0.9250 & 0.9750\\
% Specificity & 0.6897& 1.0000 & 1.0000 & 0.8696& 0.8261& 0.7391\\
% F1-Score & 0.7110& 1.0000 & 1.0000 & 0.8684& 0.9136& 0.9176\\
% AUC& 0.8181 &\textbf{1.0000} &\textbf{1.0000}& 0.9092 &\textbf{0.9380} &0.9348 \\
% \bottomrule
% \end{tabular}}
\end{table}



\subsection*{Analysis of Eumelanin category of misclassified images}

To better understand which skin tone categories are most susceptible to misclassification, we analyzed the eumelanin categories of misclassified optical images in the cooling datasets. We examined the four dark skin tone categories: Inter, InterHigh, InterLow, and InterMid. For each category, we calculated the percentage of misclassified images by comparing the number of misclassifications to the total number of images in that category within the test set. As depicted in Figure \ref{fig:eumelanin_category}, our analysis revealed that InterMid had the highest misclassification rate at about 35\%, followed by Inter at 30\%, InterHigh at approximately 25\%, and InterLow with the lowest rate at roughly 12\%. These findings indicate that InterMid images pose the greatest challenge for accurate classification, while InterLow images are the least likely to be misclassified.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth, height= 15em]{Themal_imaging_pics/GRADCAM.png}
    \caption{GRAD-CAM visualization of classifying cool, control (base) and erythema images}
    \label{fig:GRADCAM}
\end{figure*}


\subsection{Interpretability of the model}
Deep learning models are often considered 'black boxes' due to their complexity and lack of interpretability.To ensure the model's transparency, techniques like Shapley Additive explanations(SHAP)\citep{NIPS2017_7062} and  Gradient-weighted Class Activation Mapping(Grad-CAM)\citep{selvaraju2017grad} have been proprosed. To assess  where our model was looking at in making its predictions, we used GRAD-CAM.
Grad-CAM produces visual explanations for decisions made by CNN-based models. It uses the gradient of any target concept (e.g., 'cat' in a classifier) flowing into the final convolutional layer to produce a coarse localization map. This map highlights the important regions in the image for predicting the concept.
We applied Grad-CAM to visualize the regions predicted by our model for all three image modalities (optical, color thermal, and black and white thermal) in both the cooling dataset and the Erythema dataset.From the GRAD-CAM visualization, it is evident that our fine-tuned MobileNetV2 is able correctly detect the cool spot as shown in (1) and (3) in Figure\ref{fig:GRADCAM}.It is also able to correctly classify control image and detect erythema as shown in (2) and (4) respectively.

